From Electronic Design Automation to Building Design Automation: Challenges and Opportunities

Design automation, which involves the use of software tools and technologies to streamline the design process, has been widely adopted in the electronics industry, resulting in significant advancements in product development and manufacturing. However, building design, which involves the creation of complex structures and systems, has traditionally lagged behind in leveraging design automation technologies. Despite extensive research on design automation in the building industry, its application in the current design of buildings is limited. This paper aims to (1) compare the design processes between electronics and building design, (2) highlight similarities and differences in their approaches, and (3) examine challenges and opportunities associated with bringing the concept of design automation from electronics to building design.

==> background.tex <==
\section{Background}
\label{sec:background}

From design to operation, constructing a building involves several parties, including architects, engineers, building authorities, clients, financial institutions and constructors.
The integrative design guide to green building developed by Reed et al. \cite{reed2009integrative} splits the design process into nine stages: preparation, evaluation, conceptual design, schematic design, design development, construction documentation, bidding and construction, and occupants, operations, and performance feedback. 
Furthermore, they split buildings into five different subsystems: habitat, water, energy, materials, and budget. 
The integrative process involves people working on different subsystems coming together at the end of each stage to align each party's interests. 
In this paper, the energy subsystem is primarily discussed.

During the integrative design process, BIM plays an important role in retaining information from different parties during the building life cycle.
BIM was first developed in an attempt to automate and digitize hand-drawn design \cite{eastman1975use}.
It records building information such as geometry, zone layout, material properties, sensor location and data.
In recent years, the term Digital Twin (DT) has emerged.
It is defined as a virtual replica of a physical system \cite{Grieves2017}.
The BIM can act as a DT of a building that includes 3D graphical interfaces and a database for building information.
However, BIM usually doesn't have built-in energy analysis tools and often relies on other form of plug-in tools to analyze building energy performance. 
Existing BIM platforms integrate some of the BPS tools for energy analysis. 
The standard non-proprietary data exchange format for BIM are the Industry Foundation Class (IFC) \cite{IFC_iso201816739} and Green Building Extensible Markup Language (gbXML) \cite{gbxml}.
% , and Drawing Interchange Format (DXF)\cite{dxf}. 
The IFC format stores building data, including geometry, spatial elements, and sensor information. 
Construction Operations Building information exchange (COBie) \cite{COBie}, a subset of IFC,  is another data format that is becoming popular in the BIM community.
It is a model view definition of IFC and is a performance-based specification including equipment and spaces.
The gbXML format is more specifically used in energy simulation domain. 
It facilitates the exchange of data between CAD and energy analysis tools. 
However, it only takes rectangular shape for building geometry or objects, whereas the  IFC can record any shape. 
% IFC and DXF store CAD data files and gbXML can store more than 500 building components and attributes.
The data structures of the IFC, and gbXML are shown in Figure \ref{fig:datastruct}.
% DXF data format is split into different groups, whereas IFC and gbXML are structured as a hierarchy of components. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\linewidth]{figs/datastruct.png}
    \caption{Data structures for the IFC and gbXML format.}
    \label{fig:datastruct}
\end{figure}

% both formats are not yet able to represent all information across all building performance domain
% There are ongoing efforts in a variety of domains in extending both schemas to represent more information. 
The common BIM software include Autodesk Revit \cite{revit}, GraphiSoft Archicad \cite{archicad}, Bently OpenBuildings Designer (formerly AECOsim) \cite{bently} and Siemens Ecodomus \cite{Ecodomus}.
% and Gehry Technologies Digital Project \cite{DP}. 
All of the BIM software have capabilities to import or export in one or more of the standard data formats. 
Once exported, it can act as an input to the BPS tools to perform energy analysis. 
% Table \ref{table:bim} shows the common BIM software with their available exporting format and the BPS tools that are integrated into the software.
Although the communications between BIM and BPS are established, they are not yet well-developed. 
The process is not fully automatic and may require manual alteration while applying to another software. 
For example, Revit can apply thickness of a building for each material; however, EnergyPlus requires a new material input for each thickness defined \cite{calquin2014interoperability}.



% BPS tools play an important role in a building life cycle, from an early design phase to operation phase. 
% In early design phase, it helps making design choices

% \begin{table}[H]
% \caption{List of BIM platforms, available exporting format, and their connection to BPS tools.}
% \centering
% % \setlength{\tabcolsep}{0.4\tabcolsep}
% \begin{tabular}{|m{0.3\linewidth}| m{0.15\linewidth} | m{0.43\linewidth}|}
% \hline
%  \textbf{BIM}	& \textbf{Format} & \textbf{Energy Analysis Tools} \\
% \hline
% Revit (Autodesk)   & DXF, gbXML &  Insight 360, DesignBuilder, Sefaira, IES-VE, Green Building Studio \\
% \hline
% Archicad (GraphiSoft) & DXF, IFC, gbXML &   EcoDesigner Star \\
% \hline
% OpenBuildings Designer (Bently) & DXF, IFC, gbXML  & OpenBuildings Energy Simulator\\
% \hline
% EcoDomus (Siemens)& - & EnergyPlus\\
% \hline
% \end{tabular}
% \label{table:bim}
% \end{table}

% AECosim can only import IFC file but not export

% Although the communications between BIM and BPS have been addressed in several studies \cite{}, no clear design flow of BIM and BPS integration during construction process is discussed. 

% \subsection{Standard Data Exchange Methods}
% The standard data exchange between BIM and BPS are Industry Foundation Class (IFC), Green Building Extensible Markup Language (gbXML), and Data Schema File (DXF).


\subsection{Level of Detail of BIM}
The level of detail (LoD) framework of BIM is developed by the American Institute of Architects (AIA) \cite{lod_AIA}.
LoD defines the amount and degree of building information that needs to be in the BIM at different stages.
Table \ref{table:loa} describes the model information at each level. 


\begin{table}[H]
\caption{The LoD for BIM.}
\centering
\begin{tabular}{|m{0.2\linewidth}|m{0.7\linewidth}|}
\hline
 \textbf{LoD}	& \textbf{Model Descriptions} \\
\hline
LoD 100  & Approximate graphical representation of the entire building based on spatial requirements \\
\hline
LoD 200 &  Determine approximate floor plans and space boundaries (walls, elevation, and columns)  \\
\hline
LoD 300 & Detailed design for actual construction\\
\hline
LoD 400 & Precise model for fabrication, structure, electrical, mechanical, and plumbing systems\\
\hline
LoD 500 & Complete design, which represents the actual building\\
\hline
\end{tabular}
\label{table:loa}
\end{table}

The LoD framework is developed for construction purpose, and is not directly applicable to energy models. 
For example, BPS tools separate spaces into different thermal zones rather than rooms and floor plans. 
In addition, estimated occupancy schedules are one of the important factors \cite{Hong_buildsim_challenges} that affect  energy performance, but are not included as part of the model description. 
% As a result, a new level of abstraction that tailors to building energy models is needed. 
Though LoD framework has its limitations in energy models, the difference between the construction and the energy analysis purpose can be managed within the same framework.


% As a result, BPS tools were developed to model system dynamics in order to facilitate design choices. BPS tools use mathematical equations based on physical principles of buildings. 
% Details about BPS tools will be discussed in the following section. 
% With the advent of the Internet of Things (IoT), data gathering becomes easily accessible, which helps develop a more accurate model. 
% In 2012, the term Digital Twin (DT) emerged.
% It is defined as a virtual replica of a physical system \cite{Grieves2017}.
% A DT of a building can be a combination of a 3D structural model, a system dynamics model (e.g HVAC, water system), occupancy models, and the availability of renewable energy resources for grid integration. 
% In addition, it has the capability to provide real-time information on the physical building.
% In the following selection, current building modeling methods, applications, and performance metrics will be discussed. 
% Development of 


% \subsection{Building Performance Simulation}
% Building Performance Simulation (BPS), also known as building energy modeling, 

% \subsection{Data Exchange Standard}
% IFC Schema
% gbXML schema
% Data Schema File (DXF)
% IDEF Decomposition Diagram

==> graphicalabstract.tex <==
%%Graphical abstract
\begin{graphicalabstract}
\includegraphics{grabs}
\end{graphicalabstract}

==> highlights.tex <==
%%Research highlights
\begin{highlights}
\item Research highlight 1
\item Research highlight 2
\end{highlights}
